Coastal Flood Risk in the Mortgage Market: Storm Surge Models' Predictions vs. Flood Insurance Maps

Prior literature has argued that flood insurance maps may not capture the extent of flood risk. This paper performs a granular assessment of coastal flood risk in the mortgage market by using physical simulations of hurricane storm surge heights instead of using FEMA's flood insurance maps. Matching neighborhood-level predicted storm surge heights with mortgage files suggests that coastal flood risk may be large: originations and securitizations in storm surge areas have been rising sharply since 2012, while they remain stable when using flood insurance maps. Every year, more than 50 billion dollars of originations occur in storm surge areas outside of insurance floodplains. The share of agency mortgages increases in storm surge areas, yet remains stable in the flood insurance 100-year floodplain. Mortgages in storm surge areas are more likely to be complex: non-fully amortizing features such as interest-only or adjustable rates. Households may also be more vulnerable in storm surge areas: median household income is lower, the share of African Americans and Hispanics is substantially higher, the share of individuals with health coverage is lower. Price-to-rent ratios are declining in storm surge areas while they are increasing in flood insurance areas. This paper suggests that uncovering future financial flood risk requires scientific models that are independent of the flood insurance mapping process.

==> tables/aggregate_risk.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu Apr  2 17:24:47 2020
\begin{tabular}{P{2cm}P{2cm}P{2cm}P{2cm}P{2cm}}
  \hline
Loan Amount (\$) & In SFHA (\$) & Agency Amount (\$) & Agency in SFHA (\$) & Agency in SFHA (\%) \\ 
  \hline
1,386 & 134 &   826 &  79 & 9.60 \\ 
  1,848 & 177 & 1,138 & 108 & 9.50 \\ 
  2,181 & 207 & 1,375 & 131 & 9.50 \\ 
  1,930 & 190 & 1,170 & 116 & 9.90 \\ 
  1,993 & 198 & 1,100 & 112 & 10.10 \\ 
   \hline
\end{tabular}



==> tables/aggregate_risk_slr.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu Apr  2 17:32:40 2020
\begin{tabular}{P{2cm}P{2cm}P{2cm}P{2cm}P{2cm}}
  \hline
Loan Amount (b\$) & Agency Amount (b\$) & In 3 ft SLR (b\$) & Agency in 3ft SLR (b\$) & Agency in 3ft SLR (\%) \\ 
  \hline
1,386 &   826 & 23 & 11 & 49.10 \\ 
  1,848 & 1,138 & 30 & 15 & 51.30 \\ 
  2,181 & 1,375 & 35 & 18 & 52.90 \\ 
  1,930 & 1,170 & 32 & 16 & 50.60 \\ 
  1,993 & 1,100 & 33 & 15 & 46.30 \\ 
   \hline
\end{tabular}



==> tables/complex_mortgages_aggregate.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Tue Apr  7 14:18:33 2020
\begin{tabular}{p{4.5cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}}
  \hline
Mortgage Type & Total (b\$) & SFHA (b\$) & SFHA (\%) & 6ft SLR (b\$) & 6ft SLR (\%) & 3ft SLR (b\$) & 3ft SLR (\%) \\ 
  \hline
Non-Complex Mortgages & 148 & 56 & 37.60 & 64 & 43.40 & 31 & 21.10 \\ 
  Complex Mortgages &  35 & 13 & 35.40 & 15 & 42.70 &  6 & 18.10 \\ 
  Teaser Rate Mortgages &   8 &  3 & 35.90 &  3 & 43.20 &  2 & 19.80 \\ 
  Negative Amortization &   0 &  0 & 48.70 &  0 & 60.40 &  0 & 14.50 \\ 
  Interest-Only Payment &  28 & 10 & 34.70 & 12 & 42.40 &  5 & 18.20 \\ 
  Balloon Payment &  18 &  6 & 35.30 &  7 & 41.30 &  3 & 15.70 \\ 
  Other Non-Amortizing &   2 &  1 & 35.40 &  1 & 46.40 &  0 & 20.10 \\ 
   \hline
\end{tabular}



==> tables/complex_mortgages_cbsa_Boston_Cambridge_Newton__MA_NH.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu Apr 16 16:45:46 2020
\begin{tabular}{lrrrrr}
  \hline
Year & Total Loan Amount & IO & FRM & Full Documentation & NINA \\ 
  \hline
2001 & 143.17 & 2.01 & 77.01 & 53.70 & 10.08 \\ 
  2002 & 1403.20 & 183.67 & 661.19 & 224.39 & 103.31 \\ 
  2003 & 9179.79 & 949.15 & 4982.03 & 1270.23 & 619.26 \\ 
  2004 & 10434.52 & 2716.10 & 2987.78 & 1555.24 & 893.00 \\ 
  2005 & 11654.15 & 4065.04 & 3789.29 & 2781.25 & 1103.02 \\ 
  2006 & 9071.15 & 3504.98 & 4010.24 & 2500.76 & 760.32 \\ 
  2007 & 9451.02 & 3403.13 & 5709.00 & 3847.11 & 587.57 \\ 
  2008 & 5103.32 & 1217.36 & 3320.78 & 3184.45 & 11.30 \\ 
  2009 & 4702.96 & 469.37 & 3964.27 & 3010.65 & 5.65 \\ 
  2010 & 4190.80 & 486.48 & 2954.01 & 3088.16 & 13.60 \\ 
  2011 & 4370.55 & 631.69 & 2672.10 & 3480.36 & 76.43 \\ 
  2012 & 4301.39 & 712.44 & 2585.39 & 3220.19 & 15.15 \\ 
  2013 & 4723.20 & 1012.37 & 2394.87 & 3741.98 & 0.79 \\ 
  2014 & 3006.19 & 684.06 & 1255.75 & 1154.53 & 5.44 \\ 
  2015 & 5788.56 & 991.20 & 3198.88 & 1632.34 & 9.23 \\ 
  2016 & 6723.32 & 981.16 & 4094.67 & 2236.82 & 2.07 \\ 
   \hline
\end{tabular}



==> tables/complex_mortgages_cbsa_Cape_Coral_Fort_Myers__FL.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu Apr 16 16:45:46 2020
\begin{tabular}{lrrrrr}
  \hline
Year & Total Loan Amount & IO & FRM & Full Documentation & NINA \\ 
  \hline
2001 & 236.30 & 12.54 & 137.75 & 63.04 & 11.57 \\ 
  2002 & 1242.29 & 194.95 & 587.01 & 301.51 & 102.38 \\ 
  2003 & 3587.82 & 429.60 & 1800.39 & 1167.84 & 422.63 \\ 
  2004 & 4301.40 & 767.34 & 1270.47 & 1258.87 & 817.78 \\ 
  2005 & 7998.78 & 2019.19 & 2638.16 & 2235.39 & 1147.98 \\ 
  2006 & 8482.06 & 2817.84 & 3062.98 & 1937.18 & 651.82 \\ 
  2007 & 5645.10 & 2109.93 & 3136.93 & 2096.88 & 181.27 \\ 
  2008 & 1978.29 & 381.86 & 1379.30 & 1263.09 & 0.00 \\ 
  2009 & 1096.55 & 28.62 & 941.49 & 621.80 & 0.00 \\ 
  2010 & 1366.29 & 115.37 & 1067.30 & 1065.14 & 0.00 \\ 
  2011 & 1296.58 & 76.56 & 1064.06 & 963.95 & 0.00 \\ 
  2012 & 1812.23 & 163.79 & 1333.40 & 1238.64 & 8.08 \\ 
  2013 & 2246.21 & 270.04 & 1690.30 & 1587.82 & 5.36 \\ 
  2014 & 1398.25 & 123.54 & 967.49 & 538.23 & 6.10 \\ 
  2015 & 2063.57 & 150.15 & 1579.42 & 760.86 & 5.78 \\ 
  2016 & 2218.00 & 159.00 & 1730.30 & 809.76 & 0.00 \\ 
   \hline
\end{tabular}



==> tables/complex_mortgages_cbsa_Charleston_North_Charleston__SC.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu Apr 16 16:45:46 2020
\begin{tabular}{lrrrrr}
  \hline
Year & Total Loan Amount & IO & FRM & Full Documentation & NINA \\ 
  \hline
2001 & 506.99 & 20.77 & 402.93 & 162.13 & 1.49 \\ 
  2002 & 1973.66 & 142.89 & 1227.79 & 556.68 & 57.46 \\ 
  2003 & 5571.75 & 384.21 & 3339.20 & 1812.01 & 195.97 \\ 
  2004 & 5995.13 & 1009.24 & 2347.52 & 2344.96 & 167.97 \\ 
  2005 & 8602.45 & 2717.67 & 3259.83 & 2769.18 & 145.22 \\ 
  2006 & 8718.22 & 2475.66 & 3606.38 & 2786.73 & 177.61 \\ 
  2007 & 9434.66 & 3146.15 & 5572.64 & 4217.04 & 49.10 \\ 
  2008 & 4833.49 & 788.36 & 3508.89 & 2650.49 & 29.48 \\ 
  2009 & 5553.65 & 542.79 & 4421.86 & 3225.84 & 8.44 \\ 
  2010 & 4488.87 & 269.15 & 3363.17 & 3512.11 & 8.40 \\ 
  2011 & 5257.65 & 418.65 & 3699.44 & 4185.91 & 7.73 \\ 
  2012 & 5820.20 & 602.21 & 4188.64 & 4273.86 & 27.63 \\ 
  2013 & 5414.78 & 458.86 & 3862.94 & 4138.15 & 10.67 \\ 
  2014 & 3268.28 & 342.56 & 2136.03 & 1453.14 & 21.40 \\ 
  2015 & 4842.72 & 546.36 & 3301.80 & 1457.78 & 12.47 \\ 
  2016 & 4433.31 & 462.26 & 3237.37 & 1017.18 & 0.00 \\ 
   \hline
\end{tabular}



==> tables/complex_mortgages_cbsa_Miami_Fort_Lauderdale_West_Palm_Beach__FL.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu Apr 16 16:45:46 2020
\begin{tabular}{lrrrrr}
  \hline
Year & Total Loan Amount & IO & FRM & Full Documentation & NINA \\ 
  \hline
2001 & 533.86 & 33.73 & 230.85 & 131.47 & 44.59 \\ 
  2002 & 4041.33 & 532.78 & 1575.62 & 815.01 & 650.69 \\ 
  2003 & 11085.84 & 1619.13 & 4665.22 & 3248.95 & 1739.26 \\ 
  2004 & 14453.38 & 3770.87 & 3240.23 & 3492.29 & 2630.80 \\ 
  2005 & 22007.37 & 7578.29 & 4883.15 & 5318.68 & 3363.61 \\ 
  2006 & 19951.34 & 7564.57 & 6112.38 & 3835.65 & 2717.41 \\ 
  2007 & 18294.20 & 7380.61 & 8741.70 & 5401.93 & 2442.90 \\ 
  2008 & 7420.84 & 2660.07 & 3995.00 & 4503.40 & 64.52 \\ 
  2009 & 3409.29 & 770.90 & 2255.01 & 2173.94 & 0.00 \\ 
  2010 & 3819.84 & 826.03 & 2198.08 & 2886.04 & 6.54 \\ 
  2011 & 4832.58 & 1001.43 & 2619.11 & 3995.07 & 68.69 \\ 
  2012 & 8250.71 & 2136.99 & 4179.30 & 6393.28 & 30.68 \\ 
  2013 & 11367.77 & 2908.63 & 6192.96 & 8898.42 & 17.82 \\ 
  2014 & 7872.22 & 1909.24 & 3770.90 & 3258.67 & 12.46 \\ 
  2015 & 9636.89 & 2578.92 & 5223.19 & 2942.65 & 20.49 \\ 
  2016 & 8202.30 & 1850.98 & 4689.31 & 2606.46 & 16.44 \\ 
   \hline
\end{tabular}



==> tables/complex_mortgages_cbsa_New_York_Newark_Jersey_City__NY_NJ_PA.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu Apr 16 16:45:46 2020
\begin{tabular}{lrrrrr}
  \hline
Year & Total Loan Amount & IO & FRM & Full Documentation & NINA \\ 
  \hline
2001 & 3710.68 & 136.99 & 2960.38 & 711.60 & 133.45 \\ 
  2002 & 24604.07 & 2952.22 & 16159.85 & 4182.20 & 1370.35 \\ 
  2003 & 80892.55 & 7207.02 & 52178.96 & 18778.04 & 5344.79 \\ 
  2004 & 82866.09 & 17951.19 & 33498.99 & 16474.64 & 8842.21 \\ 
  2005 & 107598.28 & 36990.24 & 44297.50 & 25980.81 & 8213.02 \\ 
  2006 & 97644.53 & 41870.30 & 44156.93 & 22882.82 & 6163.28 \\ 
  2007 & 112693.27 & 54677.55 & 54337.18 & 38100.56 & 6004.80 \\ 
  2008 & 67392.74 & 25424.82 & 31518.76 & 41875.86 & 665.05 \\ 
  2009 & 42570.31 & 8681.82 & 29386.22 & 24153.42 & 305.81 \\ 
  2010 & 68114.43 & 15765.53 & 40394.67 & 49555.29 & 581.43 \\ 
  2011 & 82085.18 & 20993.14 & 40774.23 & 61872.14 & 3302.34 \\ 
  2012 & 120666.72 & 32360.23 & 56485.90 & 82498.16 & 1062.32 \\ 
  2013 & 124493.75 & 32647.94 & 61696.93 & 85340.80 & 324.79 \\ 
  2014 & 89617.40 & 20974.01 & 42539.84 & 32176.00 & 107.94 \\ 
  2015 & 124936.50 & 27023.90 & 71586.10 & 33603.96 & 183.34 \\ 
  2016 & 134703.49 & 33655.43 & 76032.81 & 33538.19 & 699.96 \\ 
   \hline
\end{tabular}



==> tables/complex_mortgages_cbsa_Portland_South_Portland__ME.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Wed Apr 15 19:38:36 2020
\begin{tabular}{rrrrrr}
  \hline
year & totalloanamount & io & fixed & total\_full\_document & nina \\ 
  \hline
2002.00 & 27.00 & 4.55 & 19.91 & 1.37 & 0.00 \\ 
  2003.00 & 309.27 & 38.60 & 241.69 & 25.42 & 0.99 \\ 
  2004.00 & 561.20 & 105.14 & 269.44 & 87.80 & 8.15 \\ 
  2005.00 & 628.75 & 112.00 & 385.36 & 195.74 & 20.85 \\ 
  2006.00 & 583.86 & 100.31 & 423.07 & 274.60 & 15.48 \\ 
  2007.00 & 622.37 & 39.58 & 528.65 & 348.77 & 16.56 \\ 
  2008.00 & 419.87 & 41.64 & 354.29 & 220.77 & 0.00 \\ 
  2009.00 & 370.02 & 10.64 & 345.34 & 251.26 & 1.40 \\ 
  2010.00 & 157.76 & 0.00 & 149.76 & 125.75 & 0.00 \\ 
  2011.00 & 122.66 & 0.00 & 92.71 & 78.65 & 0.00 \\ 
  2012.00 & 108.28 & 2.52 & 105.76 & 60.00 & 2.62 \\ 
  2013.00 & 129.57 & 16.54 & 104.71 & 78.29 & 0.00 \\ 
  2014.00 & 32.91 & 0.00 & 17.36 & 14.97 & 0.00 \\ 
  2015.00 & 305.07 & 15.64 & 248.00 & 106.17 & 0.00 \\ 
  2016.00 & 285.97 & 16.21 & 235.12 & 76.04 & 0.00 \\ 
   \hline
\end{tabular}



==> tables/complex_mortgages_cbsa_Tampa_St__Petersburg_Clearwater__FL.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu Apr 16 16:45:46 2020
\begin{tabular}{lrrrrr}
  \hline
Year & Total Loan Amount & IO & FRM & Full Documentation & NINA \\ 
  \hline
2001 & 532.69 & 3.88 & 432.12 & 163.94 & 5.40 \\ 
  2002 & 3119.11 & 355.59 & 1967.25 & 756.72 & 229.91 \\ 
  2003 & 9469.85 & 609.50 & 6196.44 & 3354.86 & 646.94 \\ 
  2004 & 9259.79 & 1743.85 & 3577.42 & 3056.86 & 1046.31 \\ 
  2005 & 14931.00 & 4650.36 & 5626.07 & 4475.17 & 1010.68 \\ 
  2006 & 14545.58 & 4075.66 & 6899.82 & 4334.05 & 627.69 \\ 
  2007 & 12787.82 & 3391.53 & 8321.51 & 5931.81 & 230.97 \\ 
  2008 & 5635.94 & 608.39 & 4386.64 & 3648.39 & 15.33 \\ 
  2009 & 4364.55 & 213.20 & 3796.27 & 2613.12 & 14.07 \\ 
  2010 & 4782.02 & 163.61 & 4189.02 & 3703.87 & 9.28 \\ 
  2011 & 5675.20 & 335.32 & 4617.16 & 4537.22 & 36.63 \\ 
  2012 & 6612.31 & 365.56 & 5542.97 & 4716.32 & 22.82 \\ 
  2013 & 8035.54 & 415.34 & 6713.54 & 5726.71 & 11.16 \\ 
  2014 & 4934.63 & 474.49 & 3525.86 & 2204.14 & 7.18 \\ 
  2015 & 6638.93 & 567.57 & 5028.80 & 2244.28 & 14.28 \\ 
  2016 & 6537.46 & 479.45 & 5129.20 & 2059.74 & 12.71 \\ 
   \hline
\end{tabular}



==> tables/complex_mortgages_cbsa_national.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Wed Apr 15 21:01:02 2020
\begin{tabular}{lrrrrr}
  \hline
Year & Total Loan Amount & IO & FRM & Full Documentation & NINA \\ 
  \hline
2012 & 168501.31 & 13732.01 & 123206.62 & 107482.46 & 1479.15 \\ 
  2013 & 169127.66 & 14365.61 & 123264.78 & 107086.27 & 644.46 \\ 
  2014 & 110067.40 & 9815.75 & 72228.05 & 41503.28 & 329.72 \\ 
  2015 & 154975.57 & 10408.84 & 117337.02 & 41563.03 & 392.62 \\ 
  2016 & 150154.66 & 9456.97 & 118730.52 & 38384.15 & 792.41 \\ 
   \hline
\end{tabular}



==> tables/complex_mortgages_national.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu Apr 16 16:49:39 2020
\begin{tabular}{cccccc}
  \hline
Year & Total Loan Amount & IO & FRM & Full Documentation & NINA \\ 
  \hline
2012 & 247,957 & 48,385 & 146,034 & 163,607 & 1,517 \\ 
  2013 & 254,336 & 51,599 & 150,428 & 170,829 &   651 \\ 
  2014 & 162,976 & 31,749 &  87,513 &  59,220 &   330 \\ 
  2015 & 237,938 & 43,204 & 147,995 &  63,267 &   391 \\ 
  2016 & 246,214 & 49,833 & 153,868 &  61,465 &   804 \\ 
  2017 & 193,332 & 37,885 & 116,386 &  54,219 & 1,068 \\ 
   \hline
\end{tabular}



==> tables/complex_mortgages_national_slosh_sfha.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Fri Apr 17 16:20:23 2020
\begin{tabular}{cccccccccc}
  \hline
Year & Total (M\$) & IO (M\$) & IO (\%) & FRM (M\$) & FRM (\%) & Full Doc. (M\$) & Full Doc. (\%) & NINA (M\$) & NINA (\%) \\ 
  \hline
2006 & 33,812 & 8,634 & 25.5\% & 14,101 & 41.7\% & 7,206 & 21.3\% & 1,714 & 5.1\% \\ 
  2007 & 22,794 & 6,325 & 27.7\% & 13,201 & 57.9\% & 6,905 & 30.3\% & 1,459 & 6.4\% \\ 
  2008 & 10,447 & 1,348 & 12.9\% &  8,068 & 77.2\% & 6,130 & 58.7\% &   357 & 3.4\% \\ 
  2009 & 10,944 &   486 &  4.4\% &  9,844 & 90.0\% & 5,738 & 52.4\% &   168 & 1.5\% \\ 
  2010 &  9,288 &   571 &  6.1\% &  7,699 & 82.9\% & 6,055 & 65.2\% &    76 & 0.8\% \\ 
  2011 &  8,194 &   816 & 10.0\% &  5,925 & 72.3\% & 5,399 & 65.9\% &   120 & 1.5\% \\ 
  2012 & 11,967 & 1,036 &  8.7\% &  9,246 & 77.3\% & 7,572 & 63.3\% &    32 & 0.3\% \\ 
  2013 & 11,460 & 1,108 &  9.7\% &  8,768 & 76.5\% & 7,247 & 63.2\% &    25 & 0.2\% \\ 
  2014 &  7,590 &   737 &  9.7\% &  5,638 & 74.3\% & 2,377 & 31.3\% &    19 & 0.2\% \\ 
  2015 & 11,567 & 1,061 &  9.2\% &  9,077 & 78.5\% & 2,346 & 20.3\% &    19 & 0.2\% \\ 
  2016 & 12,625 & 1,054 &  8.3\% & 10,344 & 81.9\% & 2,288 & 18.1\% &    17 & 0.1\% \\ 
   \hline
\end{tabular}



==> tables/reg_complex_diff_share.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Apr 03, 2020 - 04:19:48 PM
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
\\[-1.8ex] & \% IO & \% Balloon & \% Teaser & \% Neg. Amort. & \% Complex & log(Complex \$) \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 $\Delta$ \% SLR $-$ \% SFHA & $-$0.018$^{**}$ & $-$0.001$^{**}$ & $-$0.002$^{***}$ & $-$0.00003 & $-$0.018$^{***}$ & $-$0.016 \\ 
  & (0.009) & (0.001) & (0.0005) & (0.00004) & (0.002) & (0.068) \\ 
  & & & & & & \\ 
 log(Total Origination Amount) &  &  &  &  &  & 1.950$^{***}$ \\ 
  &  &  &  &  &  & (0.009) \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 71,224 & 71,224 & 71,224 & 71,224 & 71,224 & 71,224 \\ 
R$^{2}$ & 0.248 & 0.325 & 0.141 & 0.091 & 0.249 & 0.517 \\ 
Adjusted R$^{2}$ & 0.213 & 0.293 & 0.101 & 0.048 & 0.213 & 0.495 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 


==> tables/reg_complex_share_3ft_slr.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Apr 03, 2020 - 04:18:19 PM
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
\\[-1.8ex] & \% IO & \% Balloon & \% Teaser & \% Neg. Amort. & \% Complex & log(Complex \$) \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 \% Area in 3ft SLR & 0.076$^{***}$ & 0.003$^{***}$ & 0.002$^{**}$ & 0.00001 & 0.076$^{***}$ & 1.550$^{***}$ \\ 
  & (0.016) & (0.001) & (0.001) & (0.0001) & (0.004) & (0.121) \\ 
  & & & & & & \\ 
 log(Total Origination Amount) &  &  &  &  &  & 1.945$^{***}$ \\ 
  &  &  &  &  &  & (0.009) \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 71,224 & 71,224 & 71,224 & 71,224 & 71,224 & 71,224 \\ 
R$^{2}$ & 0.251 & 0.325 & 0.141 & 0.091 & 0.251 & 0.519 \\ 
Adjusted R$^{2}$ & 0.216 & 0.293 & 0.101 & 0.048 & 0.216 & 0.496 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 


==> tables/reg_complex_share_sfha.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Apr 03, 2020 - 04:18:48 PM
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
\\[-1.8ex] & \% IO & \% Balloon & \% Teaser & \% Neg. Amort. & \% Complex & log(Complex \$) \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 \% Area in SFHA & 0.033$^{***}$ & 0.002$^{***}$ & 0.002$^{***}$ & 0.00002 & 0.033$^{***}$ & 0.404$^{***}$ \\ 
  & (0.007) & (0.0005) & (0.0004) & (0.00003) & (0.002) & (0.060) \\ 
  & & & & & & \\ 
 log(Total Origination Amount) &  &  &  &  &  & 1.939$^{***}$ \\ 
  &  &  &  &  &  & (0.009) \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 72,350 & 72,350 & 72,350 & 72,350 & 72,350 & 72,350 \\ 
R$^{2}$ & 0.251 & 0.321 & 0.142 & 0.091 & 0.251 & 0.525 \\ 
Adjusted R$^{2}$ & 0.216 & 0.290 & 0.102 & 0.049 & 0.216 & 0.503 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

